Coupled Cluster con M\=oLe: Molecular Orbital Learning for Neural Wavefunctions

Density functional theory (DFT) is the most widely used method for calculating molecular properties; however, its accuracy is often insufficient for quantitative predictions. Coupled-cluster (CC) theory is the most successful method for achieving accuracy beyond DFT and for predicting properties that closely align with experiment. It is known as the ''gold standard'' of quantum chemistry. Unfortunately, the high computational cost of CC limits its widespread applicability. In this work, we present the Molecular Orbital Learning (M\=oLe) architecture, an equivariant machine learning model that directly predicts CC's core mathematical objects, the excitation amplitudes, from the mean-field Hartree-Fock molecular orbitals as inputs. We test various aspects of our model and demonstrate its remarkable data efficiency and out-of-distribution generalization to larger molecules and off-equilibrium geometries, despite being trained only on small equilibrium geometries. Finally, we also examine its ability to reduce the number of cycles required to converge CC calculations. M\=oLe can set the foundations for high-accuracy wavefunction-based ML architectures to accelerate molecular design and complement force-field approaches.

==> editing_commands.tex <==
% NOTE:
% All editing commands contain curly braces {} around them so that 
% they can easily be searched for in the final document via cmd + f.

% Highlighted comments for authors
\usepackage{soul, color}
\usepackage{multirow}
\newcommand{\Note}[1]{}
\renewcommand{\Note}[1]{#1}  % comment out this re-definition to suppress all Notes
\newcommand{\NoteSigned}[3]{{\textcolor{#2}{\Note{\textbf{[#1: #3]}}}}}
% Alternative with highlighter color rather than text colour
%\renewcommand{\NoteSigned}[3]{{\sethlcolor{#2}\Note{\hl{#1: #3}}}}

% Specific author comments
\newcommand{\pl}[1]{\NoteSigned{PL}{blue}{#1}}  % use for notes from Pietro
\newcommand{\tc}[1]{\NoteSigned{TC}{green}{#1}}
\newcommand{\cb}[1]{\NoteSigned{CB}{brown}{#1}}
\newcommand{\cj}[1]{\NoteSigned{CJ}{purple}{#1}}
\newcommand{\sm}[1]{\NoteSigned{SM}{magenta}{#1}}

% Inline todo: Flag something in the text to be done
\newcommand{\itodo}[1]{\NoteSigned{TODO}{red}{#1}}
% Preliminary: Flag preliminary statements or results
\newcommand{\prelim}[1]{\NoteSigned{Prelim}{grey}{#1}}

% Convenient other commands
\newcommand{\sowhat}{$\rightarrow$~}


% Variant of the TODO box for addressing reviewer comments
\newcommand{\bluebox}[1]{\todo[color=blue!20!white]{#1}}

